Distance-Certified Polyak-type Stepsizes for Subgradient Methods under H\"older Growth

In this paper, we consider nonsmooth convex optimization under a H{\"o}lder growth condition, with quadratic growth and weak sharp minima as two important special cases. Existing subgradient methods often employ predetermined decaying stepsize schedules, whereas the classical Polyak stepsize selects its stepsize adaptively but requires knowledge of the optimal value. We introduce a new distance-certified subgradient method (\DCSG) that follows a one-step optimization principle analogous to that underlying the Polyak stepsize, without requiring the optimal value. Specifically, \DCSG{} maintains a valid upper certificate for the current squared distance to the solution set. The method selects each stepsize by minimizing the worst-case upper bound on the next squared distance over all distances consistent with this certificate. We show that the resulting minimax problem admits a closed-form solution, yielding an explicit adaptive stepsize update. Under uniformly bounded subgradients, \DCSG{} improves upon the convergence rate of the classical subgradient method and matches the state-of-the-art rates for Lipschitz convex optimization under H{\"o}lder growth. In particular, it achieves linear convergence under sharp growth. Numerical experiments illustrate the performance of \DCSG.

==> figures/phi_table2_style.tex <==
% Shared PGFPlots style; each panel loads this inside its TikZ scope.
\definecolor{dcEndpoint}{HTML}{E53935}
\definecolor{dcSecond}{HTML}{1E88E5}

\pgfplotsset{dc table two/.style={
  width=3.55cm,height=3.55cm,scale only axis,
  at={(0,0)},anchor=south west,
  axis lines=left,axis line style={line width=0.55pt,-},
  tick align=outside,tick style={line width=0.5pt},
  tick label style={font=\scriptsize},label style={font=\small},
  xlabel={Stepsize $\alpha$},samples=241,
  ymajorgrids=true,grid style={gray!18,line width=0.3pt},
  clip=true,clip marker paths=false,
  /pgf/number format/fixed,/pgf/number format/precision=2,
  endpoint valid/.style={dcEndpoint,line width=1.15pt},
  endpoint extension/.style={dcEndpoint,densely dashed,line width=0.8pt},
  second valid/.style={dcSecond,line width=1.15pt},
  second extension/.style={dcSecond,densely dashed,line width=0.8pt},
  guide/.style={gray!65,densely dotted,line width=0.55pt,no marks},
  breakpoint/.style={only marks,mark=o,mark size=1.7pt,
    mark options={draw=gray!80,fill=white,line width=0.75pt}},
  selected/.style={only marks,mark=*,mark size=2.0pt,
    mark options={draw=black,fill=black}}
}}

